Decoding Imagined Handwriting from EEG

Patients with extreme forms of paralysis face challenges in communication, adversely impacting their quality of life. Recent studies have reported higher-than-chance performance in decoding handwritten letters from EEG signals, potentially allowing these subjects to communicate. However, all prior works have attempted to decode handwriting from EEG during actual motion. Furthermore, they assume that precise movement-onset is known. In this work, we focus on settings closer to real-world use where either movement onset is not known or movement does not occur at all, fully utilizing motor imagery. We show that several existing studies are affected by confounds that make them inapplicable to the imagined handwriting setting. We also investigate how sample complexity affects handwriting decoding performance, guiding future data collection efforts. Our work shows that (a) Sample complexity analysis in single-trial EEG reveals a noise ceiling, which can be alleviated by averaging over trials. (b) Knowledge of movement-onset is crucial to reported performance in prior works. (c) Fully imagined handwriting can be decoded from EEG with higher-than-chance performance. Taken together, these results highlight both the unique challenges and avenues to pursue to build a practical EEG-based handwriting BCI.

==> Sections/dummy.tex <==

%% Use \section commands to start a section
\section{Introduction}
\label{sec1}
%% Labels are used to cross-reference an item using \ref command.

Section text. See Subsection \ref{subsec1}.

%% Use \subsection commands to start a subsection.
\subsection{Example Subsection}
\label{subsec1}

Subsection text.

%% Use \subsubsection, \paragraph, \subparagraph commands to 
%% start 3rd, 4th and 5th level sections.
%% Refer following link for more details.
%% https://en.wikibooks.org/wiki/LaTeX/Document_Structure#Sectioning_commands

\subsubsection{Mathematics}
%% Inline mathematics is tagged between $ symbols.
This is an example for the symbol $\alpha$ tagged as inline mathematics.

%% Displayed equations can be tagged using various environments. 
%% Single line equations can be tagged using the equation environment.
\begin{equation}
f(x) = (x+a)(x+b)
\end{equation}

%% Unnumbered equations are tagged using starred versions of the environment.
%% amsmath package needs to be loaded for the starred version of equation environment.
\begin{equation*}
f(x) = (x+a)(x+b)
\end{equation*}

%% align or eqnarray environments can be used for multi line equations.
%% & is used to mark alignment points in equations.
%% \\ is used to end a row in a multiline equation.
\begin{align}
 f(x) &= (x+a)(x+b) \\
      &= x^2 + (a+b)x + ab
\end{align}

\begin{eqnarray}
 f(x) &=& (x+a)(x+b) \nonumber\\ %% If equation numbering is not needed for a row use \nonumber.
      &=& x^2 + (a+b)x + ab
\end{eqnarray}

%% Unnumbered versions of align and eqnarray
\begin{align*}
 f(x) &= (x+a)(x+b) \\
      &= x^2 + (a+b)x + ab
\end{align*}

\begin{eqnarray*}
 f(x)&=& (x+a)(x+b) \\
     &=& x^2 + (a+b)x + ab
\end{eqnarray*}

%% Refer following link for more details.
%% https://en.wikibooks.org/wiki/LaTeX/Mathematics
%% https://en.wikibooks.org/wiki/LaTeX/Advanced_Mathematics

%% Use a table environment to create tables.
%% Refer following link for more details.
%% https://en.wikibooks.org/wiki/LaTeX/Tables
\begin{table}[t]%% placement specifier
%% Use tabular environment to tag the tabular data.
%% https://en.wikibooks.org/wiki/LaTeX/Tables#The_tabular_environment
\centering%% For centre alignment of tabular.
\begin{tabular}{l|l|l}%% Table column specifiers
%% Tabular cells are separated by &
  S1 & S2 & S3 \\ %% A tabular row ends with \\
  \hline
  \hline
  4 & 5 & 6 \\
  7 & 8 & 9 \\
\end{tabular}
%% Use \caption command for table caption and label.
\caption{Table Caption}\label{fig1}
\end{table}


%% Use figure environment to create figures
%% Refer following link for more details.
%% https://en.wikibooks.org/wiki/LaTeX/Floats,_Figures_and_Captions
\begin{figure}[t]%% placement specifier
%% Use \includegraphics command to insert graphic files. Place graphics files in 
%% working directory.
\centering%% For centre alignment of image.
\includegraphics{example-image-a}
%% Use \caption command for figure caption and label.
\caption{Figure Caption}\label{fig1}
%% https://en.wikibooks.org/wiki/LaTeX/Importing_Graphics#Importing_external_graphics
\end{figure}

==> Sections/intro_old.tex <==
\section{Introduction}
\label{sec:introduction}

Patients with locked-in syndrome are unable to communicate through traditional means such as speech or writing, since their motor functions are severely impaired \citep{rousseau2013evaluation, laureys2005locked}. Brain Computer Interfaces (BCIs) that allow these subjects to communicate even in a limited fashion can significantly increase their quality of life \citep{milekovic2018stable, kubler2020history}. Many existing BCIs utilize motor imagery \citep{decety1996neurophysiological} as a control signal, which involves the subject attempting or imagining some familiar motor movement. The motor imagery paradigm is desirable as it allows for endogenous, asynchronous control, making it an ideal choice for everyday usage. Classical motor-imagery BCIs have used control signals such as left-hand/right-hand clenching, or tongue/hands/feet movement, etc \citep{mohamed2018comparison}. However, these types of control signals facilitate limited information transfer rates (ITR), and subjects must endure slow and cumbersome communication. 

Recently, imagined handwriting has produced significantly higher ITR than prior work, having been explored in the invasive setting \citep{willett2021high}. 
This previous study showed that the motor-imagery signals associated with handwriting can be reliably decoded using data from intracortical microelectrodes implanted in the precentral gyrus. In a single subject, pre-screened for high prior performance, this work demonstrated a real-time character error rate (CER) as low as 5.4\%, with a rate of communication approaching average smartphone typing speeds of the participant’s demographic. Interestingly, they found improved accuracy for letter classification than for center-out trajectories; the authors hypothesize that handwriting provides temporal as well as spatial differences in trajectories, allowing better separability of neural representations. 
% We hypothesize that this will also help with EEG-based classification of handwritten letters.
% Previous studies have sought to classify EEG activity evoked by motor imagery for cursor control and movement restoration through prosthetic limbs \cite{bright2016eeg}. 

Inspired by this work, a subsequent study \citep{pei2021online} used EEG signals to classify between the characters of “HELLO, WORLD!”, reporting an accuracy of 94\%. However, their experimental design involved writing the above characters in the same order every trial in specified boxes while looking at the tablet, shown in \ref{fig:flawed_exp_design}. Furthermore, Independent Components (ICs) representing eye-movements were not discarded from the EEG, and might be a confound. We conducted our own analysis on their data. The component shown in Fig \ref{fig:eye_IC} from ICA run on the EEG data likely represents horizontal eye movement, and was included in their predictive model. Excluding all other predictors, this artifact alone achieves 85.6\% accuracy in the classification task, while reported accuracy is 94\%. 
Thus, it appears that the reported accuracy was obtained from the model decoding the subject's horizontal eye position, rather than motor signals associated with handwriting.

\begin{figure}[h]
	\centering
	\begin{subfigure}{.3\textwidth}
		\centering
		\includegraphics[width=0.7\linewidth]{Figures/flawed_exp_design.png}
		\caption{Prior work's exp. design}
		\label{fig:flawed_exp_design}
	\end{subfigure}%
	\begin{subfigure}{.7\textwidth}
		\centering
		\includegraphics[width=0.7\linewidth]{Figures/flawed_IC.png}
		\caption{Eye IC}
		\label{fig:eye_IC}
	\end{subfigure}
	\caption{One of the 10 ICs used for prediction in prior work. The IC clearly represents the horizontal motion of the eyes tracking the letters in different boxes. This IC alone achieves 85.6\% accuracy.}
	\label{fig:prior_work}
\end{figure}


Another related work \citep{tripathi2024neuroair} attempts to decode upper-case letters traced in the air using EEG. While they achieve modest classification accuracy, a crucial difference is that only the index finger is used to trace the letter, and no hand kinematics is recorded. 

The closest related work \cite{crell2024handwritten}, similar to the one above, also captures EEG while the participant traces letters with their index finger. However, they also capture kinematics data is captured while participant's index finger traces one of 10 handwritten letters. The authors show that kinematics information can be decoded and used for 

%We hypothesize that a more naturalistic handwriting motion using the highly innervated wrist and multiple fingers will elicit stronger signals for decoding, making it a more reliable motor imagery signal. Furthermore, our experimental paradigm involved collecting the precise pen-tip velocity during handwriting, alongside the EEG recording. This allows us to uncover new insights into the trained decoder at a granular level, as well as the motor encoding of handwriting signals, discussed further in Section \ref{sec:results}. 

Both these works use index-tracing to mimic handwriting, as capturing kinematics of a single digit is easier than complex wrist motion associated with real handwriting. However, we consider that naturalistic handwriting might be better encoded in the brain compared to index-finger writing. We thus collect pen-tip kinematics using a digital pen and tablet while simultaneous EEG is recorded as the subject is performing naturalistic handwriting, allowing future analysis on the representational differences between these, if any exist.

Finally, a practical system for locked-in patients will require the ability to work with motor imagery, as in the intracortical study, rather than actual motion. While all prior work has dealt with subjects writing, we show for the first time that decoding can be done from purely imagined handwriting.

The contributions of our work are as follows:
\begin{itemize}
	\item We propose a new experimental design and collect simultaneous EEG and pen-tip velocity data under this design to evaluate the feasibility of decoding handwriting motor signals from single-trial EEG. We make this dataset publicly available.
	\item We analyze the relationship between sample complexity and EEG decoding performance for handwriting, revealing a noise ceiling that cannot be overcome simply by scaling training data.
	\item To the best of our knowledge, this work is the first to show that purely imagined handwriting can be decoded from single-trial EEG data
\end{itemize}
